Eloquent: A More Robust Transmission Scheme for LLM Token Streaming

To render each generated token in real-time for users, the Large Language Model (LLM) server generates tokens one by one and streams each token (or group of a few tokens) through the network to the user right after generation, which we refer to as LLM token streaming. However, under unstable network conditions, the LLM token streaming experience could suffer greatly from stalls since one packet loss could block the rendering of later tokens even if the packets containing them arrive on time. With a measurement study, we show that current applications suffer from increased stalls under unstable networks. For this emerging token streaming problem in LLM Chatbots that differs from previous multimedia and text applications, we propose a novel transmission scheme, called Eloquent, which puts newly generated tokens as well as currently unacknowledged tokens in the next outgoing packet. This ensures that each packet contains some new tokens and, in the meantime, is independently rendered when received, avoiding the aforementioned stalls caused by missing packets. Through simulation under various networks, we show Eloquent reduces stall ratio (proportion of token rendering wait time) by 71.0% compared to the retransmission method commonly used by real chatbot applications and by 31.6% compared to the baseline packet duplication scheme. By tailoring Eloquent to fit the token-by-token generation of LLM, we enable the Chatbots to respond like an eloquent speaker for users to better enjoy pervasive AI.

==> motivation-v1.tex <==
\tightsection{Background and Motivation}
\subsection{Token Streaming}

We provide a brief end-to-end overview of current LLM Chatbot streaming pipeline in Fig. \ref{fig:pipeline}. First, the user enters a prompt, which gets sent to the cloud data center. In the data center, the prompt is separated into tokens, which are numbers corresponding to semantic units (partial or full words). These tokens then go through a prefilling phase to be processed in parallel to understand the prompt. 
After the prefilling phase, the model iteratively predicts the next token with the current sentence, appends the token to the sentence, and repeat the process until it outputs end of sentence (EOS). In this output phase, generated tokens or the corresponding words are sent to the user through the network right after generation to provide real-time response. If the tokens were sent instead of words, they are then interpreted by the client into words. In the last step, the words are displayed on the screen in the order that they are generated. 

In this paper, we focus on the transmission of tokens (either number or corresponding word) to the client side in this token streaming pipeline. 

\tightsubsection{Current Systems under Unstable Network}

As LLM Chatbots are becoming more and more pervasive in our life, it is essentially important that the services deliver smooth experience under different network scenarios. However, network degradation, especially under wireless situations, are still frequent and could happen due to various reasons. As previous research and reports~\cite{wireless_1, wireless_2, wireless_3, wireless_4} have pointed out, packet loss under wireless situations could be due to various reasons including collision from other devices or weak signal caused by common such as a walking past a surface that blocks direct signal transmission. If users are using the LLM service under these scenarios, it is very likely that they will suffer from intermittent internet connections.

In order to learn about how current LLM Chatbot application perform under these degraded network conditions, we conducted a measurement study on one of the most popular tools to integrate LLM Chatbot into current application, ChatGPT API.

\begin{figure}
\centering
     \includegraphics[width=.99\linewidth]{figs/emulation platform.pdf}
    \caption{Our Network Emulation Setup\hanchen{make graph bigger}} 
    \label{fig:emulation}
\end{figure}



\begin{figure}
\centering
     \includegraphics[width=.99\linewidth]{figs/api.pdf}
    \tightcaption{Packet Arrival and Token Rendering of an Emulated Session of ChatGPT API \hanchen{red circle}} 
    \label{fig:api}
\end{figure}

\mypara{Measurement Testbed}
\label{emulated_measurement}
We emulated bad networking by connecting a Macbook 2023 M2 computer to hotspot of IPhone 11 using Mint LTE service in North America~\ref{fig:emulation}. Then we put the phone inside lab office and walked around outside the office (within 20m). Meanwhile on the Macbook, we started an automated bash script that repetitively start 30 conversations using same prompt and streaming option. The prompt was set to "Count to 80, with a comma between each number and no newlines. E.g., 1, 2, 3, ..." for repeating outputs. 

We record packet arrivals with tcpdump~\cite{tcpdump} with interface flag set to ``any" and extract the ChatGPT flows with IP address. To record token arrival times, we slightly modified the sample Python script provided in OpenAI documentation~\cite{openai_example}.

 
 \mypara{Findings} 
 From the packet trace, we see that the data is transmitted through encrypted TLS protocol (over TCP) and the application data protocol is HTTP.
 
Performance-wise, under this unstable network condition, compared with the reference of connecting laptop directly to high-speed wifi in office, the 95\% token rendering stall\footnote{We defined stall as inter-token gaps larger than 200ms. This follows from works in video streaming~\cite{stall1, cheng2023grace}.} increased from 377ms to 3483ms and from 1501.4ms to 2924.4ms respectively for model "GPT-3.5-turbo" and "GPT-4", under an average network loss rate of 10.5\% and 15.8\%.  

We provide a detailed analysis of a single trace to show why there is potential for 
improvement in Fig. \ref{fig:api}. As the packet arrival graphs show on the left, some packet (red-circled) were lost and retransmitted. However, the connection turned usable right after the loss and many packets containing later tokens arrived before the arrival of retransmission packets. The retransmission packets arrived much later at around 9th second due to the unstable connection. 

The impact of this "retransmission blocking future token rendering" is very severe, as shown on the right hand side. No tokens were generated from the moment these packets were lost until the retransmission came through at around 9th second. Although a lot of packets arrived after the loss, all of the tokens contained inside were blocked by the lost ones. Thus, no token was rendered during a time interval of almost 5 seconds.

\begin{figure}
\centering
     \includegraphics[width=.99\linewidth]{figs/form_fake.pdf}
    \caption{Measurement Comparison \hanchen{need to add}} 
    \label{fig:measure}
\end{figure}



\mypara{Other Applications}
We extended our measurement to other popular applications and report the qualitative results in Fig. \ref{fig:measure}. Most current applications are using TCP or QUIC protocol and uses retransmission under compromised network. This increases the stall time greatly while Claude even fail to render tokens when packet loss rates are high (but recovers when network becomes stable again).



\tightsubsection{Related Prior Work}
Although the problem of token streaming is new, there have been many prior works that aims to protect transmission against packet loss. 

The most popular method for loss-resilience is Forward Error Correction (FEC)~\cite{tambur, wicker1999reed, mackay2005fountain}. Although there are different types of coding methods including Reed-Solomon-Coding~\cite{wicker1999reed}, Fountain Coding~\cite{mackay2005fountain}, LDPC~\cite{mackay1997near}, the fundamental idea of FEC is to encode an a-byte segment to (a+b) bytes such that when any a of the (a+b) bytes arrive, the receiver can reconstruct the original data. Traditionally, the redundancy packets are added for every 10ms - 50ms interval for video and audio~\cite{blum2021webrtc, audiofec}. More recently, people have proposed a new theoretical streaming code that tries to handle burst losses and satisfy strict latency constraints for streaming applications~\cite{streaming_code, streaming_code2}. There are also some practical work on applying streaming code to audio~\cite{8057027, emara2020lowlatency} and video~\cite{tambur, 5729366}. However, it is worth noting that the latency requirement for streaming code requires a ``guard space" of guaranteed arrival after a packet loss period. Setting an accurate redundancy rates for FEC have known be extremely difficult~\cite{li2023reparo, cheng2023grace, 10.1145/3609395.3611108}. \jc{a side note: somewhere we need to call out explicitly that FEC isn't effective for token streaming since it's designed to protect a file that spans multiple packets but each token group (define it first) is much smaller than the packet size}

Besides FEC there have also been error concealment~\cite{h264_error, kang2022error} and neural-network-enhanced loss resilience methods~\cite{cheng2023grace, li2023reparo} that utilizes inter-frame and intra-frame to recover the lost part of frame. These methods usually put extra computational requirement on client end to predict the lost part. In the case of token streaming, predicting the token reliably also requires running heavy language model on client device.

\tightsubsection{Unique Properties and Challenge}
The essential problem we want to answer is: given tokens generated from the cloud and unstable network condition in the wild, how to renders the token more smoothly by the user at client side?

Comparing with the previous audio and video streaming problems, we identify the following properties for token streaming problem under unstable networks:
\begin{itemize}
    \item Increasing bitrate for transmission could not increase rendering quality.
    \item Sequence need to be strictly maintained that one lost token could block future rendering. But Video/Audios could skip frame~\cite{salsify} under loss. 
    \item The minimal operating requirement for network is much lower since text data are much smaller than audio (100Kbps) and video (1Mbps).
\end{itemize}

Given these properties, we claim that a robust token streaming protocol should be able to deliver packets smoothly even under consistently unstable network. More specifically, it should prevent the problem of lost packet blocking rendering for subsequent arrived tokens since retransmission packets could arrive much later due to unstable connection. This could be done by adding redundancy without causing quality drop. However, traditional redundancy sytems using methods like FEC fall short since they assume network is only temporarily unstable and would often cause retransmission as shown later in \S\ref{protocol:example}. 

